Uniform Convergence of Gradients for Non-Convex Learning and Optimization

We investigate 1) the rate at which refined properties of the empirical risk---in particular, gradients---converge to their population counterparts in standard non-convex learning tasks, and 2) the consequences of this convergence for optimization. Our analysis follows the tradition of norm-based capacity control. We propose vector-valued Rademacher complexities as a simple, composable, and user-friendly tool to derive dimension-free uniform convergence bounds for gradients in non-convex learning problems. As an application of our techniques, we give a new analysis of batch gradient descent methods for non-convex generalized linear models and non-convex robust regression, showing how to use any algorithm that finds approximate stationary points to obtain optimal sample complexity, even when dimension is high or possibly infinite and multiple passes over the dataset are allowed. Moving to non-smooth models we show----in contrast to the smooth case---that even for a single ReLU it is not possible to obtain dimension-independent convergence rates for gradients in the worst case. On the positive side, it is still possible to obtain dimension-independent rates under a new type of distributional assumption.

==> nips_style.tex <==
% !TEX root = paper.tex

%\usepackage{geometry}
% \usepackage[letterpaper, left=1in, right=1in, top=1in, bottom=1in]{geometry}

\usepackage[dvipsnames,table]{xcolor}
\usepackage[colorlinks=true, linkcolor=Blue, citecolor=Blue]{hyperref}
\usepackage{microtype}

% From nips template
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography


\usepackage{natbib}
\setcitestyle{square, comma, numbers, sort & compress}
\bibliographystyle{plainnat}
%\usepackage{natbib}
%\bibliographystyle{plainnat}
%\bibpunct{(}{)}{;}{a}{,}{,}

\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{bbm}
\usepackage{amsfonts}
\usepackage{amssymb}
\let\vec\undefined
\usepackage{MnSymbol} %Actually conflicts with amssymb and others

\usepackage{xpatch}

%%% theorems

\theoremstyle{definition}  %Sets style of subsequent newtheorems to 'definition'
\newtheorem{exercise}{Exercise}
\newtheorem{claim}{Claim}
\newtheorem{lemma}{Lemma}
%\newtheorem{assumption}{Assumption}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{fact}{Fact}
%\newtheorem{model}{Model}
%\newtheorem{problem}{Problem}
\newtheorem{assumption}{Assumption}
\newtheorem{problem}{Problem}
\newtheorem{model}{Model}
\theoremstyle{plain}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}

\xpatchcmd{\proof}{\itshape}{\normalfont\proofnameformat}{}{}
\newcommand{\proofnameformat}{\bfseries}

\newcommand{\notimplies}{\nRightarrow}

%%% prettyref

\usepackage{prettyref}
\newcommand{\pref}[1]{\prettyref{#1}}
\newcommand{\pfref}[1]{Proof of \prettyref{#1}}
\newcommand{\savehyperref}[2]{\texorpdfstring{\hyperref[#1]{#2}}{#2}}
\newrefformat{eq}{\savehyperref{#1}{\textup{(\ref*{#1})}}}
\newrefformat{eqn}{\savehyperref{#1}{Equation~\ref*{#1}}}
\newrefformat{tab}{\savehyperref{#1}{Table~\ref*{#1}}}
\newrefformat{lem}{\savehyperref{#1}{Lemma~\ref*{#1}}}
\newrefformat{def}{\savehyperref{#1}{Definition~\ref*{#1}}}
\newrefformat{thm}{\savehyperref{#1}{Theorem~\ref*{#1}}}
\newrefformat{fact}{\savehyperref{#1}{Fact~\ref*{#1}}}
\newrefformat{corr}{\savehyperref{#1}{Corollary~\ref*{#1}}}
\newrefformat{sec}{\savehyperref{#1}{Section~\ref*{#1}}}
\newrefformat{app}{\savehyperref{#1}{Appendix~\ref*{#1}}}
\newrefformat{ass}{\savehyperref{#1}{Assumption~\ref*{#1}}}
\newrefformat{ex}{\savehyperref{#1}{Example~\ref*{#1}}}
\newrefformat{fig}{\savehyperref{#1}{Figure~\ref*{#1}}}
\newrefformat{alg}{\savehyperref{#1}{Algorithm~\ref*{#1}}}
\newrefformat{rem}{\savehyperref{#1}{Remark~\ref*{#1}}}
\newrefformat{conj}{\savehyperref{#1}{Conjecture~\ref*{#1}}}
\newrefformat{prop}{\savehyperref{#1}{Proposition~\ref*{#1}}}
\newrefformat{proto}{\savehyperref{#1}{Protocol~\ref*{#1}}}
\newrefformat{prob}{\savehyperref{#1}{Problem~\ref*{#1}}}
\newrefformat{claim}{\savehyperref{#1}{Claim~\ref*{#1}}}

==> section_deeper.tex <==
% !TEX root = paper.tex

\subsection{Further tools}
\dfcomment{switch this stuff to work on $z$s}

For a scalar-valued function class $\cF$, we let $\rad_{\cF}(\xr[n]) = \En_{\eps}\sup_{f\in\cF}\sum_{t=1}^{n}\eps_{t}f(x_t)$. When $\cF$ is $\bbR^{K}$-valued, we define two different Rademacher complexities: $\rad^{\ls_{p}}(\cF\midsem\xr[n]) = \En_{\eps}\sup_{f\in\cF}\nrm*{\sum_{t=1}^{n}\eps_{t}f(x_t)}_{p}$ and $\radvec(\cF\midsem\xr[n]) = \En_{\mb{\eps}}\sup_{f\in\cF}\sum_{t=1}^{n}\tri*{\mb{\eps}_{t}, f(x_t)}$.

\begin{definition}
For any $\bbR^{K}$-valued function class $\cF$, let $\cN_{p, \nrm*{\cdot}}(\cF, \veps, \xr[n])$, denote the size of the smallest set $V\subseteq{}\bbR^{n\times{}K}$ such that
\[
\max_{f\in\cF}\min_{v\in{}V}\prn*{\frac{1}{n}\sum_{t=1}^{n}\nrm*{f(x_t)-v_t}^{p}}^{1/p} \leq{} \veps.
\]
For $\ls_{q}$ norms we overload this notation via $\cN_{p, q}(\cF, \veps, \xr[n]) = \cN_{p, \nrm*{\cdot}_{q}}(\cF, \veps, \xr[n])$.
\end{definition}
The most important covering number in our analyses wll be $\cN_{2,2}$.

Dudley's entropy integral and Sudakov's partial converse are two standard theorems used to relate Rademacher complexity of a function class to its empirical metric entropy from above and below. Here we use two variants adapted to handle vector-valued function classes.

Vector-valued covers of the $2,2$ type we use here were a key component of the analysis of \cite{bartlett2017spectrally}. The theorems below establish that these vector-valued covers and the vector-valued Rademacher averages $\radvec$ are equivalent up to logarithmic factors. While this follows from standard techniques, it does not appear to have been known in the literature.

\begin{theorem}[Dudley]
  \label{thm:dudley_vector}
  For any function class $\cF\subseteq{}\cX\to\bbR^{K}$,
  \begin{equation}
    \radvec(\cF\midsem\xr[n]) \leq{} \inf_{\alpha>0}\crl*{
      4\alpha{}n\sqrt{K} + 12\sqrt{n}\int_{\alpha}^{\mathrm{rad}_{2,2}(\cF\midsem{}\xr[n])}\sqrt{\log\cN_{2,2}(\cF,\veps,\xr[n])}d\veps
      },
\end{equation}
where $\mathrm{rad}_{2,2}(\cF\midsem\xr[n])\ldef{}\min\crl*{\veps\mid{}\cN_{2,2}(\cF,\veps,\xr[n])=1}$.
\end{theorem}
Note that $\mathrm{rad}_{2,2}(\cF\midsem{}\xr[n])\leq{}\sup_{f\in\cF}\max_{t\in\brk*{n}}\nrm*{f(x_t)}_{2}$, since $\crl*{\mb{0}}$ always serves as a cover at this scale.

\begin{theorem}[Sudakov]
  \label{thm:sudakov_vector}
For any class $\cF\subseteq{}\cX\to\bbR^{K}$, data sequence $\xr[n]$ with $\radvec(\cF\midsem\xr[n])\geq{}1$, for any precision $\veps>0$,
\begin{equation}
\log\cN_{2,2}(\cF, \veps, \xr[m]) \leq{} \frac{c_{n,K}}{n}\cdot\prn*{\frac{\radvec(\cF\midsem\xr[n])}{\veps}}^{2},
\end{equation}
where $c_{n,K} = O(\log{}(nK))$.
The cover may be assumed to be proper without loss of generality.
\end{theorem}

\dfcomment{Explain: hope this tools will be useful in the future even though we have poor understanding of optimization. optimization is out of scope.}
\dfcomment{quickly explain intuition behind the proof and covering etc. if space.}

This section is specialized to euclidean geometry to avoid making what is already a notationally heavy analysis even more cumbersome.

\begin{theorem}
  \dfcomment{Generalization for computational graphs}
\end{theorem}

\begin{theorem}
NN gradient and hessian.
\end{theorem}

\begin{theorem}
Linear network (via tengyu's paper)?
\end{theorem}

\begin{theorem}[Deep \dfcomment{?} ReLU networks]
\dfcomment{worst case: Just do the $\ls_{1}$ weight bounded version.}  
\end{theorem}

\begin{theorem}[Hierarchical clustering]

\end{theorem}

\paragraph{Discussion and related work}
The proof technique in this section builds on the technique of \cite{bartlett2017spectrally}, and indeed theorem \pref{thm:todo} recovers this result for the case of feedforward networks. While many new generalization bounds have been proposed since that paper appeared, to our knowledge none of these results improve over \cite{bartlett2017spectrally} under the same assumptions \cite{neyshabur2017exploring, neyshabur2017pac, arora2018stronger, golowich2017size} (see discussion in \cite{bartlett2017spectrally}, NIPS version). Nonetheless, we certainly do not expect \pref{thm:todo} to be tight for arbitrary function classes, and understanding when the bound can be improved is an exciting direction for future research. We are hopeful that the basic computational graph abstraction can be combined with alternative proof techniques such as those of \cite{golowich2017size}, which offer weaker dependence on depth (in our case, number of paths?) at the cost of worse dependence on $n$.

\ascomment{Montenari Models fall through, Gradient and Hessian for Neural networks} 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> section_experiments.tex <==
Experiments for deeper models.
\begin{itemize}
\item Phi for SGD with original vs. random labels.
\item (Hopefully) some sort of SGD vs. FGD separation.
\item randomized MNIST with FGD and SGD 
\item Counter-Data, Good-Data margin plots
\end{itemize}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> section_optimization.tex <==
Broader picture for writing: We want to move toward stronger \emph{algorithm-dependent} generalization results for nonconvex stochastic optimization.

\begin{itemize}
\item Basic convergence results given optimization routines stated in the Montanari paper .
\item Contrast with SGD-type methods: Eg: \citep{ge2015escaping}. Running \cite{jin2017escape} for our setting instead should give better dimension dependence. \dfcomment{todo: See if jin paper actually applies here.} Note that if we take more than one pass over the dataset on a function with population strict saddle, it's not obvious if it will even converge to a local minimum on the empirical loss a-priori, since you may not have empirical strict saddle.
\item Escaping saddle points with finite sum structure: \cite{jin2017escape, allenzhu2017natasha2, allenzhuli2017neon2}
\item SGD-type methods \citep{ghadimi2013stochastic,ghadimi2016accelerated} work with multiple passes.
\item Other related work: \cite{hardt2016train} (very weak)
\item For cases where we don't have good optimization results: \citep{davis2018stochastic,davis2018smooth}
\item Specialized algorithms for sum-of-nonconvex, Maybe also cool even for smooth: \citep{reddi2016proximal, allenzhu2018katyushax, allenzhuli2017neon2, allenzhu2017natasha2} with multiple passes etc.
\end{itemize}

\subsection{Functions with the ??? property}

\subsection{Strongly morse functions}

\dfcomment{strongly morse theorem, corollaries (GD converges in...)...}
\begin{lemma}
  \dfcomment{Generalized version of montanari theorem 2: ``given gradient and hessian convergence, we get...''}
\end{lemma}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper.tex"
%%% End:

